Nearby Early-Type Galactic Nuclei at High Resolution: Dynamical Black Hole and Nuclear Star Cluster Mass Measurements

We present a detailed study of the nuclear star clusters (NSCs) and massive black holes (BHs) of four of the nearest low-mass early-type galaxies: M32, NGC205, NGC5012, and NGC5206. We measure dynamical masses of both the BHs and NSCs in these galaxies using Gemini/NIFS or VLT/SINFONI stellar kinematics, Hubble Space Telescope (HST) imaging, and Jeans Anisotropic Models. We detect massive BHs in M32, NGC5102, and NGC5206, while in NGC205, we find only an upper limit. These BH mass estimates are consistent with previous measurements in M32 and NGC205, while those in NGC5102 and NGC5206 are estimated for the first time, and both found to be $<$$10^6~M_{\odot}$. This adds to just a handful of galaxies with dynamically measured sub-million $M_{\odot}$ central BHs. Combining these BH detections with our recent work on NGC404's BH, we find that 80\% (4/5) of nearby, low-mass ($10^9-10^{10}~M_{\odot}$; $\sigma_{\star}\sim20-70$ km/s) early-type galaxies host BHs. Such a high occupation fraction suggests the BH seeds formed in the early epoch of cosmic assembly likely resulted in abundant seeds, favoring a low-mass seed mechanism of the remnants, most likely from the first generation of massive stars. We find dynamical masses of the NSCs ranging from $2-80\times10^6~M_{\odot}$ and compare these masses to scaling relations for NSCs based primarily on photometric mass estimates. Color gradients suggest younger stellar populations lie at the centers of the NSCs in three of the four galaxies (NGC205, NGC5102, and NGC5206), while the morphology of two are complex and are best-fit with multiple morphological components (NGC5102 and NGC5206). The NSC kinematics show they are rotating, especially in M32 and NGC5102 ($V/\sigma_{\star}\sim0.7$).

==> astromacro.tex <==
\usepackage{color}
\usepackage{graphicx}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Lyman series lines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ly}{Lyman}
\newcommand{\Lya}{\mbox{Ly$\alpha$}}
\newcommand{\lya}{\mbox{Ly$\alpha$}}
\newcommand{\lyb}{\mbox{Ly$\beta$}}
\newcommand{\lyg}{\mbox{Ly$\gamma$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\kms}{\mbox{km s$^{-1}$}}
\newcommand{\cmm}{\mbox{cm$^{-2}$}}
\newcommand{\cmmm}{\mbox{cm$^{-3}$}}
\newcommand{\escsh}{$\mathrm{ergs}
        \mathrm{\ s}^{-1}
        \mathrm{\ cm}^{-2}
        \mathrm{\ sr}^{-1}
        \mathrm{\ Hz}^{-1}$}
\newcommand{\hmpc}{\mbox{$h^{-1}$Mpc}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Light elements
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\het}{\mbox{$^3$He}}
\newcommand{\hef}{\mbox{$^4$He}}
\newcommand{\lisv}{\mbox{$^7$Li}}
\newcommand{\lisx}{\mbox{$^6$Li}}
\newcommand{\yp}{\mbox{Y$_p$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Cosmological  Parameters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ETA}{\mbox{$\eta $}}
\newcommand{\ob}{\mbox{$\Omega_b$}}
\newcommand{\obh}{\mbox{$\Omega_bh^{2}$}}
\newcommand{\om}{\mbox{$\Omega_m$}}
\newcommand{\ol}{\mbox{$\Omega_{\Lambda } $}}
\newcommand{\sig}{\mbox{$\sigma_8$}}
\newcommand{\gammahe}{\mbox{$\gamma_{228}$}}
\newcommand{\gammah}{\mbox{$\gamma_{912}$}}
\newcommand{\jnu}{\mbox{$J_{\nu }$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Parameters Measured 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\zabs}{\mbox{$z_{\rm abs}$}}
\newcommand{\chisq}{\mbox{$\chi^2$}}
\newcommand{\nhi}{\mbox{N$_{\rm H I}$}}
\newcommand{\lnhi}{\mbox{log \nhi}}
\newcommand{\ndi}{\mbox{N$_{\rm D I}$}}
\newcommand{\lndi}{\mbox{log \ndi}}
\newcommand{\bhi}{\mbox{$b_{\rm H I}$}}
\newcommand{\zdh}{\mbox{$z = 2.526$}}
\newcommand{\zdhvalue}{2.526}
\newcommand{\da}{\mbox{$D_a$}}
\newcommand{\fbar}{\mbox{$\bar{F}$}}
\newcommand{\pdff}{\mbox{flux distribution}}
\newcommand{\bsig}{\mbox{$b_{\sigma}$}}
\newcommand{\pl}{\mbox{$P_{-2}$}}
\newcommand{\pmed}{\mbox{$P_{-1.5}$}}  
\newcommand{\ps}{\mbox{$P_{-1}$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Misc
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\etal}{{\it et al.}}
\newcommand{\lyaf} {\lya\ forest}
\newcommand{\mf}{\mbox{$10^{-5}$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The following defines commands to leave messages in draft copies of the
%% document.  The messages will only be visible if draftmode=true.  
%% \documentclass[11pt,preprint]{aastex}
%% \input{astronomy-commands}
%% \draftmodeptrue  or \draftmodepfalse
%% Note that
%% I use plain old TeX if's instead of Latex's \ifthenelse because the TeX
%% version can be imbedded into Latex commands (such as \section).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\ifdraftmodep
\draftmodepfalse

\newcommand{\NOTE}[1]{\ifdraftmodep {\color {red} [{\it #1}]} \fi}
\newcommand{\DONE}[1]{\ifdraftmodep {\color {blue} [DONE: {\it #1}]} \fi}
\newcommand{\RESP}[1]{\ifdraftmodep {\color {blue} {\it #1}} \fi}

%\newcommand{\NB}[1]{\ifdraftmodep {\color {red} [NB: {\it #1}]} \fi}
% Rahman Amanullah
\newcommand{\RA}[1]{\ifdraftmodep {\color {red} [RA: {\it #1}]} \fi}
% Kyle Barbary
\newcommand{\KB}[1]{\ifdraftmodep {\color {red} [KB: {\it #1}]} \fi}
% Kyle Dawson
\newcommand{\KD}[1]{\ifdraftmodep {\color {red} [KD: {\it #1}]} \fi}
% Alex Gude
\newcommand{\AG}[1]{\ifdraftmodep {\color {red} [AG: {\it #1}]} \fi}
% Saul Perlmutter
\newcommand{\SP}[1]{\ifdraftmodep {\color {red} [SP: {\it #1}]} \fi}
% David Rubin
\newcommand{\DR}[1]{\ifdraftmodep {\color {red} [DR: {\it #1}]} \fi}
% Tony Spadafora
\newcommand{\ALS}[1]{\ifdraftmodep {\color {red} [ALS: {\it #1}]} \fi}
% Nao Suzuki
\newcommand{\NS}[1]{\ifdraftmodep {\color {red} [NS: {\it #1}]} \fi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Define a boolean to indicate if this should be set with emulateapj
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifapjp
\apjpfalse

